LoRA-IR: Taming Low-Rank Experts for Efficient All-in-One Image Restoration

Prompt-based all-in-one image restoration (IR) frameworks have achieved remarkable performance by incorporating degradation-specific information into prompt modules. Nevertheless, handling the complex and diverse degradations encountered in real-world scenarios remains a significant challenge. To tackle this, we propose LoRA-IR, a flexible framework that dynamically leverages compact low-rank experts to facilitate efficient all-in-one image restoration. Specifically, LoRA-IR consists of two training stages: degradation-guided pre-training and parameter-efficient fine-tuning. In the pre-training stage, we enhance the pre-trained CLIP model by introducing a simple mechanism that scales it to higher resolutions, allowing us to extract robust degradation representations that adaptively guide the IR network. In the fine-tuning stage, we refine the pre-trained IR network through low-rank adaptation (LoRA). Built upon a Mixture-of-Experts (MoE) architecture, LoRA-IR dynamically integrates multiple low-rank restoration experts through a degradation-guided router. This dynamic integration mechanism significantly enhances our model's adaptability to diverse and unknown degradations in complex real-world scenarios. Extensive experiments demonstrate that LoRA-IR achieves SOTA performance across 14 IR tasks and 29 benchmarks, while maintaining computational efficiency. Code and pre-trained models will be available at: https://github.com/shallowdream204/LoRA-IR.

==> fig/visual_udc.tex <==
\begin{figure*}[t]
	% \captionsetup{font=small}
	
	\centering
	
	\newcommand{\h}{0.105}
	\newcommand{\wa}{0.12}
	\newcommand{\wb}{0.16}
	\newcommand{\g}{-0.7mm}
	\setlength\tabcolsep{1.4pt}
  	\renewcommand{\arraystretch}{1}
	\resizebox{1.00\linewidth}{!} {
			\renewcommand{\h}{0.143}
			\newcommand{\w}{0.22}
				\begin{adjustbox}{valign=t}
					\begin{tabular}{cccccc}
						\includegraphics[height=\h \textwidth, width=\w \textwidth]{fig/visual_results/udc/lq_box.jpg} \hspace{\g} &
						\includegraphics[height=\h \textwidth, width=\w \textwidth]{fig/visual_results/udc/lq_crop.jpg} \hspace{\g} &
				\includegraphics[height=\h \textwidth, width=\w \textwidth]{fig/visual_results/udc/promptir_crop.jpg} \hspace{\g} &
				\includegraphics[height=\h \textwidth, width=\w \textwidth]{fig/visual_results/udc/diffuir_crop.jpg} \hspace{\g} &
				\includegraphics[height=\h \textwidth, width=\w \textwidth]{fig/visual_results/udc/ours_crop.jpg} \hspace{\g} &
      			\includegraphics[height=\h \textwidth, width=\w \textwidth]{fig/visual_results/udc/gt_crop.jpg} 
						\\
						 LQ Image \hspace{\g} &
						Input \hspace{\g} &
						PromptIR~\cite{promptir}\hspace{\g} &
      					DiffUIR~\cite{diffuir} &
                 		\textbf{LoRA-IR (Ours)} &
                            GT \hspace{\g}
						\\
					\end{tabular}
				\end{adjustbox}
			
	}
 %  	\renewcommand{\arraystretch}{1}
	% \resizebox{1.00\linewidth}{!} {
	% 		\renewcommand{\h}{0.163}
	% 		\newcommand{\w}{0.22}
	% 			\begin{adjustbox}{valign=t}
	% 				\begin{tabular}{cccccc}
	% 					\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/5de_real/1/lq_box.jpg} \hspace{\g} &
	% 					\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/5de_real/1/lq_crop.png} \hspace{\g} &
	% 			\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/5de_real/1/promptir_crop.png} \hspace{\g} &
 %      			\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/5de_real/1/diffuir_crop.png} \hspace{\g} &
 %               	\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/5de_real/1/ours_crop.png} \hspace{\g} &
	% 			\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/5de_real/1/gt_crop.png} 
	% 					\\
	% 					Blurry Image \hspace{\g} &
	% 					Input \hspace{\g} &
	% 					PromptIR\hspace{\g} &
 %      					DiffUIR \hspace{\g} &
 %      					\textbf{LoRA-IR} \hspace{\g} &
 %                            GT \hspace{\g}
	% 					\\
	% 				\end{tabular}
	% 			\end{adjustbox}
			
	% }

 %  	\renewcommand{\arraystretch}{1}
	% \resizebox{1.00\linewidth}{!} {
	% 		\renewcommand{\h}{0.163}
	% 		\newcommand{\w}{0.22}
	% 			\begin{adjustbox}{valign=t}
	% 				\begin{tabular}{cccccc}
	% 					\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/1/input_box2.png} \hspace{\g} &
	% 					\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/1/input2_crop.png} \hspace{\g} &
	% 			\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/1/trans2_crop.png} \hspace{\g} &
 %      			\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/1/wgws2_crop.png} \hspace{\g} &
 %               	\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/1/ours2_crop.png} \hspace{\g} &
	% 			\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/1/gt2_crop.png} 
	% 					\\
	% 					Snowy Image \hspace{\g} &
	% 					Input \hspace{\g} &
	% 					Transweather\hspace{\g} &
 %      					WGWS \hspace{\g} &
 %      					\textbf{LoRA-IR} \hspace{\g} &
 %                            GT \hspace{\g}
	% 					\\
	% 				\end{tabular}
	% 			\end{adjustbox}
			
	% }

 %   	\renewcommand{\arraystretch}{1}
	% \resizebox{1.00\linewidth}{!} {
	% 		\renewcommand{\h}{0.163}
	% 		\newcommand{\w}{0.22}
	% 			\begin{adjustbox}{valign=t}
	% 				\begin{tabular}{cccccc}
	% 					\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/2/input_box3.png} \hspace{\g} &
	% 					\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/2/input3_crop.png} \hspace{\g} &
	% 			\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/2/trans3_crop.png} \hspace{\g} &
 %      			\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/2/wgws3_crop.png} \hspace{\g} &
 %               	\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/2/ours3_crop.png} \hspace{\g} &
	% 			\includegraphics[height=\h \textwidth, width=\w \textwidth]{visual/aw/2/gt3_crop.png} 
	% 					\\
	% 					Hazy Image \hspace{\g} &
	% 					Input \hspace{\g} &
	% 					Transweather\hspace{\g} &
 %      					WGWS \hspace{\g} &
 %      					\textbf{LoRA-IR} \hspace{\g} &
 %                            GT \hspace{\g}
	% 					\\
	% 				\end{tabular}
	% 			\end{adjustbox}
			
	% }
 \vspace{-0.2cm}
	\caption{\textbf{[Setting \Rmnum{4}]} Visual results on TOLED~\cite{udc} for \textbf{\textit{training-unseen tasks generalization evaluation}}. Zoom in for a better view.}
 \vspace{-0.4cm}
	\label{fig:visual_udc}
\end{figure*}
